Interleaving classical and reversible

Given a simple recursive function, we show how to extract two interacting processes from it. The two processes can be described by means of iterative programs, one of which is intrinsically reversible, in a language that, up to minor details, belongs to the core of widely used imperative programming languages. We implement the two processes as interleaving synchronous JAVA threads whose interaction is equivalent to the recursive function they are extracted from.

==> yarel.tex <==
\section{\textsf{Yarel}}
\label{section:Yarel}
We introduce \textsf{Yarel} by commenting on the definition of a set of functions that we can see as the core of an arithmetic library \verb|ArithNat|.
Section~\ref{section:The grammar of Yarel formally} contains the grammar that defines \textsf{Yarel}.

%%%
\subsection{Built-in functions and modules}
Being \textsf{Yarel} a paradigmatic domain specific language designed after the introduction of the class \textsf{RPP} of Reversible Primitive Permutations \cite{PaoliniPiccoloRoversi:RPP}, it makes available a set of primitive basic functions. They are \verb|id|, \verb|inc|, \verb|dec|, \verb|neg| and any finite permutation \verb|\$ i_1 \ldots i_n\!$\| where $ i_1 \ldots i_n$ are the first $ n $ elements of $ \mathbb{N} $.

The \emph{identity} \verb|id| has arity 1. It leaves its argument unchanged.  Formally:
\begin{prooftree}
	\AxiomC{}
	\RightLabel{$ \scriptsize \textsc{id} $}
	\UnaryInfC{$ \mbox{\verb|id|}\, [x : v] \downarrow [x : v ] $}
\end{prooftree}
whose conclusion formalizes the relation $ \downarrow $ between the input 
$ [x : v ] $ on its left-hand side and $ [x : v] $ on its right-hand side, mediated by \verb|id| itself. Every $ [x : v] $ is a finite function that associates a value $ v $ to $ x $, the single argument of \verb|id|. 
We \emph{line} or \emph{port} the name $ x $.

The \emph{negation} \verb|neg| has arity 1. It negates the value of a given port:
\begin{prooftree}
	\AxiomC{}
	\RightLabel{$ \scriptsize \textsc{neg} $}
	\UnaryInfC{$ \mbox{\verb|neg|}\, [x : v] \downarrow [x : -v] $}
\end{prooftree}

The \emph{increment} \verb|inc| has arity 1. It increments the value of a given port:
\begin{prooftree}
	\AxiomC{}
	\RightLabel{$ \scriptsize \textsc{inc} $}
	\UnaryInfC{$ \mbox{\verb|inc|}\, [x : v] \downarrow [x : v+1] $}
\end{prooftree}

The \emph{decrement} \verb|dec| has arity 1. It decrements the value of a given port:
\begin{prooftree}
	\AxiomC{}
	\RightLabel{$ \scriptsize \textsc{dec} $}
	\UnaryInfC{$ \mbox{\verb|dec|}\, [x : v] \downarrow [x : v-1] $}
\end{prooftree}

A \emph{permutation} \verb|\$i_1 \ldots i_n\!$\| has arity $ n \geq 1 $. 
It associates the value of the $ i_1 $-th input port to the first output port,
the value of the $ i_2 $-th input port to the second output port, and so on:
\begin{prooftree}
\AxiomC{$ \{1 \ldots n\} = \{i_1 \ldots i_n\} $}
\RightLabel{$ \scriptsize \chi $}
\UnaryInfC{$ \mbox{\verb|\\ $i_1 \ldots i_n\!$\\ |} \, 
	[x_{1} : v_1, \ldots, x_{n} : v_n]
	\downarrow 
	[x_{1} : v_{i_1}, \ldots, x_{n} : v_{i_n}]$}
\end{prooftree}
\noindent
For example, the transposition is:
\begin{prooftree}
	\AxiomC{$ $}
	\RightLabel{$ \scriptsize \chi $}
	\UnaryInfC{$ \mbox{\verb|\\2 1\\ |} \, 
		[x : u, y : v] \downarrow [x : v, y : u]$}
\end{prooftree}

\textsf{Yarel} allows to organize its functions by means of modules:
\begin{lstlisting}[language=yarel]
/** Convention: ModuleName.rl must be the name of the file 
  * that contains this module. Every word in a composite 
  * name should start with a capital letter.
  */
module ModuleName {
  import ModuleNameParent0.*
  DOTS
  import ModuleNameParentN.*
  // Body of the module goes here.
}
\end{lstlisting}
The directive \verb|import| allows to organize modules as a direct acyclic graph.

%%%%%%%%%%%
\subsection{The module \verb|ArithNat|.}
For our introductory purpose, we define the module \verb|ArithNat| with the 
four basic arithmetic functions \verb|sum|, \verb|mul(tiplication)|, 
\verb|quo(tient)| and \verb|sub(traction)| in it. Every of them is committed to 
produce the correct output if applied to values of $ \mathbb{N} $ only.
We introduce \verb|sum|, \verb|mul(tiplication)|, \verb|quo(tient)| and 
\verb|sub(traction)| in that order to simplify the simultaneous 
description of the operational semantics of \textsf{Yarel}.

%%%%
\subsubsection{The function \verb|sum|}
Its natural definition is:
\begin{lstlisting}
//////// sum	
dcl sum : 2 int
/* in : $u$, $v$
 * out: $u+v$, $v$
 * Iterates inc as many times as $ v $, starting from $ u $.
 */
def sum := it[inc]
\end{lstlisting}
\noindent
By the \emph{declaration} \verb|dcl|, the function \verb|sum| has input and output arity 2, i.e. it takes two integers as input, as specified by the \emph{type} 
\verb|2 int|, and gives two integers as output. An equivalent, syntactically legal, declaration is \verb|dcl sum : int, int|.

The \emph{definition} \verb|def sum := it[inc]| says that \verb|sum| iterates the function \verb|inc|. 

The definition of \verb|sum| makes it evident that the programs of \textsf{Yarel} are pointless. We define them by composing combinators without any reference to their input or output ports. We explicitly mention ports and the associated values at the level of the operational semantics only.

%%%
\subsubsection{The iteration \verb|it[$ f $]|}
If $ f $ is a function of \textsf{Yarel} with arity $ n \geq 1$, then 
\verb|it[$ f $]| has arity $ n+1 $. The value $ v $ of the $ n+1 $-th input port controls the length of the iteration. Three rules define the operational semantics of \verb|it[$ f $]|:
\begin{prooftree}
\AxiomC{$  $}
\RightLabel{$ \scriptsize \textsc{itz}$}
\UnaryInfC{$\mbox{\verb|it[$f$]|}
	(\Delta \cdot [x : 0])
	\downarrow 
	\Delta' \cdot [x : 0]$}
\end{prooftree}
\begin{prooftree}
\AxiomC{$ v > 0 $}
\AxiomC{$\mbox{\verb+($ f $|dec);it[$f$]+}
	(\Delta \cdot [x : v]) 
	\downarrow \Delta' \cdot [x : v']$}
\RightLabel{$ \scriptsize \textsc{its}$}
\BinaryInfC{$\mbox{\verb|it[$f$]|}
	(\Delta \cdot [x : v])
	\downarrow 
	\Delta'\cdot [x : v]$}
\end{prooftree}
\begin{prooftree}
\AxiomC{$ v < 0 $}
\AxiomC{$\mbox{\verb+($ f $|inc);it[$f$]+}
	(\Delta \cdot [x : v]) 
	\downarrow \Delta' \cdot [x : v']$}
\RightLabel{$ \scriptsize \textsc{its}$}
\BinaryInfC{$\mbox{\verb|it[$f$]|}
	(\Delta \cdot [x : v])
	\downarrow 
	\Delta' \cdot [x : v]$}
\end{prooftree}
In them, $ \Delta\cdot [x : v] $ is the concatenation between the two finite functions $ \Delta $ and $ [x : v] $ under the assumption that their domains $ \operatorname{dom}(\Delta) $ and $ \{x\} $ are disjoint. Like in $ [x : v]$, the function $ \Delta $ associates values $ v_1,\ldots, v_n $ to the ports $ x_1, \ldots, x_n $, respectively, for some $ n \geq 1 $.
The cardinality $ |\operatorname{dom}(\Delta)| $ of $ \operatorname{dom}(\Delta) $ and the arity of $ f $ must coincide in every of the above rules.
The rule \textsc{itz} says that $ \mbox{\verb|it[$ f $]|} $ is the identity on the whole $ \Delta\cdot [x : v] $ if $ v $ is equal to $ 0 $.
The rule \textsc{itg} inductively applies $ \mbox{\verb|it[$ f $]|} $ to the result of $ f $ applied to $ \Delta $, if $ v > 0 $, and simultaneously decreases the value associated to $ x $ to assure the termination.
Analogously, the rule \textsc{its} inductively applies $ \mbox{\verb|it[$ f $]|} $ to the result of $ f $ applied to $ \Delta $, if $ v < 0 $ and simultaneously increases the value associated to $ x $ to assure the termination.

For example, let us assume we want to sum 1 and 2. We have:
\begin{center}
%\hspace{-1cm}
\scalebox{.9}{
 \begin{minipage}{\linewidth}
  \begin{prooftree}
  	\AxiomC{$ \Phi_0 $}
  	\noLine
  	\UnaryInfC{$\mbox{\verb+(inc|dec)+}\, 
  		[x:1, y:2]\downarrow [x:2, y:1]
  		$}
 
  	\AxiomC{$ \Psi $}
  	\noLine
    \UnaryInfC{$\mbox{\verb|it[inc]|}[x:2, y : 1] \downarrow [x:3, y:1] $}
    
  	\RightLabel{$ \scriptsize \textsc{seq}$}
  	\BinaryInfC{$\mbox{\verb+(inc|dec);it[inc]+}[x:1, y:2] \downarrow [x:3, y:1]$}
  	
  	\RightLabel{$ \scriptsize \textsc{itg}$}
    \UnaryInfC{$\mbox{\verb|it[inc]|}[x:1, y:2] \downarrow [x:3, y:2]$}
  \end{prooftree}
 \end{minipage}
}
\end{center}
where $ \Psi $ is:
\begin{center}
%	\hspace{-1cm}
	\scalebox{.9}{
		\begin{minipage}{\linewidth}
			\begin{prooftree}
				\AxiomC{$ \Phi_1 $}
				\noLine
				\UnaryInfC{$\mbox{\verb+(inc|dec)+}\, 
					[x:2, y:1]\downarrow [x:3, y:0] $}
				
				\AxiomC{$ $}
				\RightLabel{$ \scriptsize \textsc{itz}$}
				\UnaryInfC{$\mbox{\verb|it[inc]|}[x:3, y : 0] \downarrow [x:3, y:0] $}
				
				\RightLabel{$ \scriptsize \textsc{seq}$}
				\BinaryInfC{$\mbox{\verb+(inc|dec);it[inc]+}
					[x:2, y : 1] \downarrow [x:3, y:0] $}
				
				\RightLabel{$ \scriptsize \textsc{itg}$}
				\UnaryInfC{$\mbox{\verb|it[inc]|}[x:2, y : 1] \downarrow [x:3, y:1] $}
			\end{prooftree}
		\end{minipage}
	}
\end{center}
\noindent
and both $ \Phi_0, \Phi_1$ are the obvious derivations.

%%%
\subsubsection{Sequential composition}
An alternative description of how an iteration of \textsf{Yarel} works passes through the \emph{sequential composition}. If $ f $ and $ g $ are two functions of \textsf{Yarel} with identical arity $ n $, and $ |\operatorname{\Delta}| = n $, for some $ \Delta $, we can use them one after the other:
\begin{prooftree}
\AxiomC{$ f\,\Delta \downarrow \Delta'   $}
\AxiomC{$ g\,\Delta' \downarrow \Delta'' $}
\RightLabel{$ \scriptsize \textsc{seq} $}
\BinaryInfC{$\mbox{\verb|($f$;$g$)|}\, \Delta \downarrow \Delta'' $}
\end{prooftree}

It follows that the application of \verb|sum| to $ [x : 1, y : 5] $, i.e. the application of \verb|it[inc]| to $ [x : 1, y : 5] $, is equivalent to the sequential composition:
\begin{align*}
&\mbox{\verb|inc;inc;inc;inc;inc|}
\end{align*}
with as many occurrences of \verb|inc| as the value associated to $ y $.

%%%%
\subsection{The function \verb|mul(tiplication)|} 
A natural definition is:
\begin{lstlisting}
//////// multiplication	
dcl mul : 3 int
/* in : $u$, $v$, $a$
 * out: $a+u+\ldots+u$, $u$, $v$ 
 *           where $u+\ldots+u$ has $v$ occurrences of $u$
 * Iterates sum as many times as $v$, using the value of the 
 * ancilla $a$ as a starting point
 */
def mul := \3 1 2\;it[sum] 
\end{lstlisting}
\noindent
It sequentially composes a permutation and an iteration of \verb|sum|. 
As an example we build the derivation that computes $ 3 \times 2 $. 
Considered its typographical dimension we introduce it piecewise.
Its conclusion is: 
\begin{center}
\hspace{-2cm}
\scalebox{.8}{
    \begin{minipage}{\textwidth}
        \begin{prooftree}
            \AxiomC{$  $}
            \RightLabel{$ \scriptsize \chi$}            \UnaryInfC{$\mbox{\verb|\\3 1 2\\|}\,
                [x:3, y:2, a:0] 
                \downarrow 
                [x:0, y:3, a:2]$}
            
            \AxiomC{$\Phi_1$}
            \noLine
            \UnaryInfC{$\mbox{\verb|it[sum]|}
                [x:0, y:3, a:2] 
                \downarrow 
                [x:6, y:3, a:2]$}
            
            \RightLabel{$ \scriptsize \textsc{seq}$}
            \BinaryInfC{$\mbox{\verb|\\3 1 2\\;it[sum]|}\,
                [x:3, y:2, a:2] 
                \downarrow 
                [x:6, y:3, a:2]$}
        \end{prooftree}
    \end{minipage}
}
\end{center}
It takes care of sequentially composing the permutation \verb|\3 1 2\| and the iteration \verb|it[sum]|.
The first unfolding in $ \Phi_1 $ is:
\begin{center}
\hspace{-2cm}
\scalebox{.8}{
 \begin{minipage}{\textwidth}
  \begin{prooftree}
    \AxiomC{$ \Psi_1 $}
    \noLine
    \UnaryInfC{$\mbox{\verb+(sum|dec)+}\,
         [x:3, y:0, a:2] \downarrow 
         [x:3,y:3, a:1] $}
    
    \AxiomC{$ \Phi_2$}
    \noLine
    \UnaryInfC{$\mbox{\verb|it[sum]|}
         [x:3, y:3, a:1] \downarrow 
         [x:6, y:3, a:2] $}
    
    \RightLabel{$ \scriptsize \textsc{seq}$}
    \BinaryInfC{$\mbox{\verb+(sum|dec);it[sum]+}
               [x:0, y:3, a:2] 
               \downarrow 
               [x:6, y:3, a:2]$}
    
    \RightLabel{$ \scriptsize \textsc{itg}$}
    \UnaryInfC{$\mbox{\verb|it[sum]|}
	            [x:0, y:3, a:2] 
            	\downarrow 
             	[x:6, y:3, a:2]$}

  \end{prooftree}
 \end{minipage}
}
\end{center}
with $ \Psi_1 $:
\begin{center}
	\hspace{-1.5cm}
	\scalebox{.8}{
		\begin{minipage}{\textwidth}
			\begin{prooftree}
				\AxiomC{$ \Psi_2 $}
				\noLine
				\UnaryInfC{$\mbox{\verb|it[inc]|}\,
					[x:0,y:3]\downarrow [x:3,y:3]\ $}
				\RightLabel{$ \scriptsize \textsc{fcall}$}
				\UnaryInfC{$\mbox{\verb|sum|}\,
					[x:0,y:3]\downarrow [x:3,y:3]\ $}
				
				\AxiomC{$  $}
				\RightLabel{$ \scriptsize \textsc{dec}$}
				\UnaryInfC{$\mbox{\verb|dec|}\,
					[a:2]\downarrow [a:1]\ $}
				
				\RightLabel{$ \scriptsize \textsc{par}$}
				\BinaryInfC{$\mbox{\verb+(sum|dec)+}\,
					[x:3, y:0, a:2] \downarrow 
					[x:3,y:3, a:1] $}
			\end{prooftree}
		\end{minipage}
	}
\end{center}
\noindent
The occurrence of $ \textsc{fcall}$ in $ \Psi_1 $ relies on the assumption that a \emph{look-up table} $ \Gamma $ exists which associates names of functions to the corresponding body, in accordance with definitions \verb|def| and declarations \verb|dcl| already met in the module:
\begin{prooftree}
\AxiomC{$ \Gamma(f)\,\Delta \downarrow \Delta'$}
\RightLabel{$ \scriptsize \textsc{fcall}$}
\UnaryInfC{$f\,\Delta \downarrow \Delta'  $}
\end{prooftree}
\noindent
So, from the conclusion of $ \textsc{fcall} $ to its assumption, the 
definition \verb|it[inc]| replaces \verb|sum|. Of coourse, an analogous replacement takes place in $ \Phi_2 $.

%%%
\subsection{The function \verb|quo(tient)|}
Let us suppose we want to compute the quotient of dividing 8 by 3 in \textsf{Yarel}. To that purpose we implement the algorithm that distributes the 8 unities in groups of 3 elements until the reminder, initially set to 8, is left with less than 3 elements.
The number of distributions is the quotient. Ideally, it is necessary to iterate the subtraction of the value 3 from 8 as many times as 2. The point is that the iteration of \textsf{Yarel} needs to know the value 2 in advance to work properly, but it is exactly the number we must discover, given 8 and 3.

The solution is to iterate a function --- we call it \verb|dis(tribution)Step| --- as many times as 8, or, more generally, as the value \verb|D| of the dividend. The goal of \verb|disStep| is essentially to subtract 3, or, more generally, the value \verb|d| of the divisor, from the value \verb|r| of the reminder. Meanwhile, \verb|disStep| counts the number of subtractions, i.e. it stepwise discovers the value \verb|q| of the quotient.
As soon as \verb|r| becomes negative, \verb|disStep| must stop counting. We achieve this behavior by incrementing the value \verb|n(egative)o(verflow)c(ounter)| whenever \verb|r| assumes a negative value.. The definition of \verb|disStep| is:
\begin{lstlisting}
dcl disStep : 4 int 
/* in : $r$(eminder), $d$(ivisor), $q$(otient), 
                       $n$(egative)$o$(verflow)$c$(ounter)
 * out: $r'$, $d'$, $q'$, $noc'$
 * disStep stands for `distribution step'.
 * disStep is part of the definition of quo(tient).
 * disStep takes $d$ elements from what remains to be 
 * distributed in $r$ and counts a new distribution 
 * round in $q$, when possible. The distribution is 
 * forbidden by positive values of $noc$ which counts 
 * the attempts to distribute more that what remains 
 * in $r$. The value of $noc$ becomes positive as soon as 
 * the difference $r-d$ becomes negative.
 */
def disStep :=  (sub|inc|id)
               ;\2 3 4 1\
               ;(id|disSel)
               ;\4 1 2 3\
\end{lstlisting}
\noindent
It is the sequential composition of four programs.
The first one is the \emph{parallel composition} \verb+sub|inc|id+ 
of the functions \verb|sub(tractrion)|, \verb|inc| and \verb|id|.

We shall define \verb|sub| in Section~\ref{subsection:The function subtraction}.
For the moment, suffice it to say that it has arity 2. If applied to
$ [x:u, y:v] $ yields $ [x:u-v,  y:v] $:
\begin{prooftree}
	\AxiomC{$  $}
	\RightLabel{$ \scriptsize \textsc{sub}$}
	\UnaryInfC{$\mbox{\verb|sub|}\,[x:u, y:v]
		\downarrow [x:u-v, y:v]$}
\end{prooftree}
\noindent

A parallel composition works as follows:
\begin{prooftree}
\AxiomC{$ f\, \Delta_f \downarrow \Delta'_f$}
\AxiomC{$ g\, \Delta_g \downarrow \Delta'_g $}
\RightLabel{$ \scriptsize \textsc{par} $}
\BinaryInfC{$\mbox{\verb+($f$|$g$)+}\, (\Delta_f \cdot \Delta_g) 
	\downarrow 
	\Delta'_f \cdot \Delta'_g$}
\end{prooftree}
i.e. the interpretations of $ f $ and $ g $ are independent one from the other.
The aim of \verb|sub| in \verb+sub|inc|id+ is to subtract $ d $ from $ r $. \
The role of \verb|inc| counts that subtraction.
Once \verb|\2 3 4 1\| rearranges the list of values
$ r, d, q, noc $ as $ d, q, noc, r $ they become the values that the parallel composition \verb+id|disSel+ takes as its input. 
In it, \verb|id| leaves the divisor unchanged.
The definition of \verb|dis(tribution)Sel(ection)| is:
\begin{lstlisting}
dcl disSel: 3 int
/* in : $q $, $noc $, $r $
 * out: $q'$, $noc'$, $r'$
 * disSel stands for `distribution selection'.
 * It is a selection tree that decides which 
 * between $ q $ and $ noc $ to leave unchanged, 
 * depending on the value of $ r $.
 */
 def disSel := if[if[id  //// $ q $   if $ noc > 0$ (impossible)
                    ,id  //// $ q $   if $ noc = 0$
                    ,id  //// $ q $   if $ noc < 0$ (impossible)
                    ];(id|id)  // $ q $, $ noc $   if $ r-d > 0$
                 ,if[id  //// $ q $   if $ noc > 0 $ (impossible)
                    ,id  //// $ q $   if $ noc = 0 $
                    ,id  //// $ q $   if $ noc < 0 $ (impossible)
                    ];(id|inc) // $ q $, $ noc+1 $ if $ r-d = 0 $
                 ,if[dec //// $ q-1 $ if $ noc > 0 $
                    ,dec //// $ q-1 $ if $ noc = 0 $
                    ,id  //// $ q $   if $ noc < 0 $ (impossible)
                    ];(id|inc) // $ q $, $ noc+1 $ if $ r-d < 0 $
                 ]
\end{lstlisting}
\noindent
It is a selection tree that nests instances of the \emph{selection} 
\verb|if[$ g $,$ z $,$ s $]| with the following operational semantics:
\begin{prooftree}
\AxiomC{$ v > 0 $}
\AxiomC{$ g\, \Delta \downarrow \Delta' $}
\RightLabel{$ \scriptsize \textsc{ifg} $}
\BinaryInfC{$\mbox{\verb|if[$g$,$z$,$s$]|}
	(\Delta \cdot [x : v]) 
	\downarrow 
	\Delta' \cdot [x : v]$}
\end{prooftree}
\begin{prooftree}
\AxiomC{$ z\, \Delta \downarrow \Delta' $}
\RightLabel{$ \scriptsize \textsc{ifz}$}
\UnaryInfC{$\mbox{\verb|if[$g$,$z$,$s$]|}
	(\Delta \cdot [x : 0]) 
	\downarrow 
	\Delta' \cdot [x : 0]$}
\end{prooftree}
\begin{prooftree}
\AxiomC{$ v < 0 $}
\AxiomC{$ s\, \Delta \downarrow \Delta' $}
\RightLabel{$ \scriptsize \textsc{ifs} $}
\BinaryInfC{$\mbox{\verb|if[$g$,$z$,$s$]|}
	(\Delta \cdot [x : v]) 
	\downarrow 
	\Delta' \cdot [x : v]$}
\end{prooftree}
\noindent
The comments in the source of \verb|disSel| show how the corresponding branch alters $ q $ and $ noc $, and which is the condition that activates that branch. The value $ r $ of the reminder selects the branch of the outer selection and value $noc$ of the ``negative overflow'' selects the branch of the selected innermost selection. We leave $ q $ as \verb|disSel| receives it whenever $ r $ is non negative and $ noc $ is zero.
However, we start increasing $ noc $ as soon as $r$ is no more strictly positive. We necessarily decrease $ q $ that \verb|disSel| takes in input whenever $ r $ is strictly negative and $ noc $ positive.
The reason is that we anyway increase $q$ before knowing if this is an acceptable action, i.e. before calling \verb|disSel|.

Let us focus again on \verb|disStep|. Its last step \verb|\4 1 2 3\| reorganizes the values to let them ready for a further application of \verb|disStep| itself, if required.

For example, starting from $ [x_1:8, x_2:3, x_3:0, x_4:0] $,
i.e. $ r = 8, d = 3, q = 0$ and $ noc = 0 $, the 8-times iteration of \verb|disStep| yields the following sequence of
configurations:
\begin{equation}
\label{equation:list of configurations by disStepIteration8div3}
\begin{tabular}{lccc}
$[x_1:  5,$ &$x_2:3,$ &$x_3:1,$ &$x_4:0]$\\
$[x_1:  2,$ &$x_2:3,$ &$x_3:2,$ &$x_4:0]$\\
$[x_1: -1,$ &$x_2:3,$ &$x_3:2,$ &$x_4:1]$\\
$[x_1: -4,$ &$x_2:3,$ &$x_3:2,$ &$x_4:2]$\\
$[x_1: -7,$ &$x_2:3,$ &$x_3:2,$ &$x_4:3]$\\
$[x_1:-10,$ &$x_2:3,$ &$x_3:2,$ &$x_4:4]$\\
$[x_1:-13,$ &$x_2:3,$ &$x_3:2,$ &$x_4:5]$\\
$[x_1:-16,$ &$x_2:3,$ &$x_3:2,$ &$x_4:6]$
\end{tabular}
\end{equation}
\noindent
In the second configuration, $ x_1 $ contains the reminder value $ 2 $, which is smaller than the value of the dividend in $ x_2 $ and the correct value of the quotient in $ x_3 $. All the configurations that follow never change the value of the quotient in $ x_3 $, but keep subtracting the dividend from the hypothetical reminder, while $ noc $ in $ x_4 $ increases.

We are finally in the position to define \verb|quo(tient)|.
It must iterate \verb|disStep| as many times as the value $ D $. We define 
\verb|quo| as:
\begin{lstlisting}
//////// quotient
dcl quo : 5 int
/* in : $D$(ividend), $d$(ivisor), $q$(otient), 
          $i$(teration unfolder), $n$(egative)$o$(verflow)$c$(ounter)
 * out: $r'$, $d$, $q'$, $i'$, $noc'$
 * quo(tient) gives the quotient of $ D/d $.
 */
def quo :=  \4 1 2 3 5\
           ;(sum|id|id|id) 
           ;\2 3 4 5 1\ 
           ;it[disStep]
\end{lstlisting}
\noindent
The assumption is to apply \verb|quo| to $[x_1:D, x_2:d, x_3:0, x_4:0, x_5:0]$.
We need two copies of $ D $. One serves as initial value of the reminder. 
The other is the number of unfolding of \verb|it[disStep]|.
We obtain those two copies by first applying \verb|\4 1 2 3 5\|:
\begin{center}
\hspace{-1cm}
\scalebox{.85}{
\begin{minipage}{\textwidth}
\begin{prooftree}
  \AxiomC{$ $}
  \RightLabel{$ \scriptsize \chi$}
  \UnaryInfC{$\mbox{\verb|\\4 1 2 3 5\\|}\,
    [x_1:D, x_2:d, x_3:0, x_4:0, x_5:0]
	\downarrow 
	[x_1:0, x_2:D, x_3:d, x_4:0, x_5:0]$
  }
\end{prooftree}
\end{minipage}
}
\end{center}
\noindent
and then using \verb|sum|:
\begin{center}
	\hspace{-1cm}
	\scalebox{.85}{
		\begin{minipage}{\textwidth}
			\begin{prooftree}
				\AxiomC{$\Phi$}
				\noLine
				\UnaryInfC{$\mbox{\verb+(sum|id|id|id)+}
					[x_1:0, x_2:D, x_3:d, x_4:0, x_5:0]
					\downarrow 
					[x_1:D, x_2:D, x_3:d, x_4:0, x_5:0]$}
			\end{prooftree}
		\end{minipage}
	}
\end{center}
The effect of the further permutation \verb|\2 3 4 5 1\| is:
\begin{center}
	\hspace{-1cm}
	\scalebox{.85}{
		\begin{minipage}{\textwidth}
			\begin{prooftree}
				\AxiomC{$ $}
				\RightLabel{$ \scriptsize \chi$}
				\UnaryInfC{$\mbox{\verb|\\2 3 4 5 1\\|}\,
					[x_1:D, x_2:D, x_3:d, x_4:0, x_5:0]
					\downarrow 
					[x_1:D, x_2:d, x_3:0, x_4:0, x_5:D]$
				}
			\end{prooftree}
		\end{minipage}
	}
\end{center}
\noindent
In it $ [x_1:D, x_2:d, x_3:0, x_4:0, x_5:D] $ has $ x_5 $ ready to drive the $ D $-long iteration of \verb|disStep| whose input will correctly be
$ [x_1:D, x_2:d, x_3:0, x_4:0] $.

%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
	\centering
	\scalebox{.9}{
		\begin{tabular}{c}
			\\[1mm]
			\AxiomC{}
			\RightLabel{$ \scriptsize \textsc{id} $}
			\UnaryInfC{$ \mbox{\verb|id|}\, [x : v] \downarrow [x : v ] $}
			\DisplayProof			
			\qquad
			\AxiomC{}
			\RightLabel{$ \scriptsize \textsc{neg} $}
			\UnaryInfC{$ \mbox{\verb|neg|}\, [x : v] \downarrow [x : -v] $}
			\DisplayProof			
			\\[0.7cm]
			\AxiomC{}
			\RightLabel{$ \scriptsize \textsc{dec} $}
			\UnaryInfC{$ \mbox{\verb|dec|}\, [x : v] \downarrow [x : v-1] $}
			\DisplayProof			
			\qquad
			\AxiomC{}
			\RightLabel{$ \scriptsize \textsc{inc} $}
			\UnaryInfC{$ \mbox{\verb|inc|}\, [x : v] \downarrow [x : v+1] $}
			\DisplayProof			
			\\[0.7cm]
			\AxiomC{$ \{1 \ldots n\} = \{i_1 \ldots i_n\} $}
			\RightLabel{$ \scriptsize \chi $}
			\UnaryInfC{$ \mbox{\verb|\\ $ i_1 \ldots i_n\!$\\|}\,
				[x_{1} : v_1, \ldots, x_{n} : v_n]
				\downarrow 
				[x_{1} : v_{i_1}, \ldots, x_{n} : v_{i_n}]$}
			\DisplayProof			
			\\[0.7cm]
			\AxiomC{$ \Delta\, f\, \Delta'   $}
			\AxiomC{$ \Delta'\, g\, \Delta'' $}
			\RightLabel{$ \scriptsize \textsc{seq} $}
			\BinaryInfC{$\Delta\, \mbox{\verb|($f$;$g$)|}\, \Delta'' $}
			\DisplayProof			
			\qquad
			\AxiomC{$ \Delta_f\, f\,  \Delta'_f$}
			\AxiomC{$ \Delta_g\, g\,  \Delta'_g $}
			\RightLabel{$ \scriptsize \textsc{par} $}
			\BinaryInfC{$(\Delta_f \cdot \Delta_g)\, \mbox{\verb+($f$|$g$)+}\,  
				(\Delta'_f \cdot \Delta'_g)$}
			\DisplayProof			
			\\[0.7cm]
			\AxiomC{$ v > 0 $}
			\AxiomC{$ g\, \Delta \downarrow \Delta' $}
			\RightLabel{$ \scriptsize \textsc{ifg} $}
			\BinaryInfC{$\mbox{\verb|if[$g$,$z$,$s$]|}
				(\Delta \cdot [x : v]) 
				\downarrow 
				\Delta' \cdot [x : v]$}
			\DisplayProof			
			\\[0.7cm]
			\AxiomC{$ z\, \Delta \downarrow \Delta' $}
			\RightLabel{$ \scriptsize \textsc{ifz}$}
			\UnaryInfC{$\mbox{\verb|if[$g$,$z$,$s$]|}
				(\Delta \cdot [x : 0]) 
				\downarrow 
				\Delta' \cdot [x : 0]$}
			\DisplayProof			
			\\[0.7cm]
			\AxiomC{$ v < 0 $}
			\AxiomC{$ s\, \Delta \downarrow \Delta' $}
			\RightLabel{$ \scriptsize \textsc{ifs} $}
			\BinaryInfC{$\mbox{\verb|if[$g$,$z$,$s$]|}
				(\Delta \cdot [x : v]) 
				\downarrow 
				\Delta' \cdot [x : v]$}
			\DisplayProof			
			\\[0.7cm]



\AxiomC{$ v > 0 $}
\AxiomC{$(\Delta \cdot [v])\  \mbox{\verb+($ f $|dec);it[$f$]+}\
	 (\Delta' \cdot [v'])$}
\RightLabel{$ \scriptsize \textsc{its}$}
\BinaryInfC{$(\Delta \cdot [v])\ \mbox{\verb|it[$f$]|}\
(\Delta'\cdot [v])$}
            \DisplayProof			
            \\[1cm]
\AxiomC{$  $}
\RightLabel{$ \scriptsize \textsc{itz}$}
\UnaryInfC{$(\Delta \cdot [0])\ \mbox{\verb|it[$f$]|}\
	(\Delta' \cdot [0])$}
            \DisplayProof			
            \\[0.7cm]
\AxiomC{$ v < 0 $}
\AxiomC{$(\Delta \cdot [v])\ \mbox{\verb+($ f $|inc);it[$f$]+}\
	(\Delta' \cdot [v'])$}
\RightLabel{$ \scriptsize \textsc{its}$}
\BinaryInfC{$(\Delta \cdot [v])\ \mbox{\verb|it[$f$]|}\
	(\Delta' \cdot [v])$}
            \DisplayProof			
            \\[0.7cm]
			\AxiomC{$ \Gamma(f)\,\Delta \downarrow \Delta'$}
			\RightLabel{$ \scriptsize \textsc{fcall}$}
			\UnaryInfC{$f\,\Delta \downarrow \Delta'  $}
			\DisplayProof			
			\\[0.25cm]
		\end{tabular}
	}
	\caption{The single-relation big-step operational semantics of 
		\textsf{Yarel} that defines the behavior of any program not subject to 
		\verb|inv|.}
	\label{figure:Single-relation big-step operational semantics of Yarel: 
		first part}
\end{figure}

\subsection{Operational semantics: a first part}
For ease of reference, Figure~\ref{figure:Single-relation big-step operational 
semantics of Yarel: first part} collects the whole set of rules we have introduced so far to define \verb|sum|, \verb|mul| and \verb|quo|.
The coming definition of \verb|sub| will be the ``excuse'' complete the introduction of the whole operational semantics of \textsf{Yarel}. 

%%%
\subsection{The function \verb|sub(traction)| and the operator \verb|inv|}
\label{subsection:The function subtraction}
The natural definition of \verb|sub| is:
\begin{lstlisting}
//////// subtraction	
dcl sub : 2 int
/* in : $x$, $y$
 * out: $x-y$, $y$
 * Eventually iterates dec on $x$ as many times as $y$.
 * Behaviour achieved by inverting sum, 
 * i.e. by iterating the inverse of inc
 */
def sub := inv[sum]
\end{lstlisting}
\noindent
Like for \verb|sum|, the function \verb|sub| has input and output arity 2.
The \emph{definition} \verb|def sub := inv[sum]| applies the operator 
\verb|inv| to the previously defined function \verb|sum|. This defines 
\verb|sub| as the \emph{inverse} of \verb|sum|. 


%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
	\centering
	\scalebox{.9}{
		\begin{tabular}{c}
			\AxiomC{$ \mbox{\verb|id|}\, \Delta \downarrow \Delta' $}
			\RightLabel{$ \scriptsize \textsc{i-id} $}
			\UnaryInfC{$ \mbox{\verb|inv[id]|}\, \Delta \downarrow \Delta' $}
			\DisplayProof			
			\qquad
			\AxiomC{$ \mbox{\verb|neg|}\, \Delta \downarrow \Delta' $}
            \RightLabel{$ \scriptsize \textsc{i-neg} $}
            \UnaryInfC{$ \mbox{\verb|inv[neg]|}\, \Delta \downarrow \Delta' $}
            \DisplayProof			
			\\[0.7cm]
			\AxiomC{$ \mbox{\verb|inc|}\, \Delta \downarrow \Delta' $}
			\RightLabel{$ \scriptsize \textsc{i-dec} $}
			\UnaryInfC{$ \mbox{\verb|inv[dec]|}\, \Delta \downarrow \Delta' $}
			\DisplayProof			
			\qquad
			\AxiomC{$ \mbox{\verb|dec|}\, \Delta \downarrow \Delta' $}
			\RightLabel{$ \scriptsize \textsc{i-inc} $}
			\UnaryInfC{$ \mbox{\verb|inv[inc]|}\, \Delta \downarrow \Delta' $}
			\DisplayProof			
			\\[0.7cm]
			\AxiomC{$ \{1 \ldots n\} = \{i_1 \ldots i_n\} $}
			\RightLabel{$ \scriptsize \textsc{i-}\chi $}
			\UnaryInfC{$ \mbox{\verb|inv[\\$i_1\ldots i_n\!$\\]|}\, 
				[x_{1} : v_1, \ldots, x_{n} : v_n]
				\downarrow 
				[x_{i_1} : v_{1}, \ldots, x_{i_n} : v_{n}]$}
			\DisplayProof			
			\\[0.7cm]
			\AxiomC{$ g\,\Delta \downarrow \Delta'   $}
			\AxiomC{$ f\,\Delta' \downarrow \Delta'' $}
			\RightLabel{$ \scriptsize \textsc{i-seq} $}
			\BinaryInfC{$\mbox{\verb|inv[$ f $;$ g $]|}\, 
				\Delta \downarrow \Delta'' $}
			\DisplayProof			
			\qquad
			\AxiomC{$ \mbox{\verb|inv[$ f $]|}\, \Delta_f \downarrow \Delta'_f$}
			\AxiomC{$ \mbox{\verb|inv[$ g $]|}\, \Delta_g \downarrow \Delta'_g 
				$}
			\RightLabel{$ \scriptsize \textsc{i-par} $}
			\BinaryInfC{$\mbox{\verb+inv[$f$|$g$]+}\, 
				(\Delta_f \cdot \Delta_g) 
				\downarrow 
				\Delta'_f \cdot \Delta'_g$}
			\DisplayProof			
			\\[0.7cm]
			\AxiomC{$\mbox{\verb|if[inv[$ g $],inv[$ z $],inv[$ s $]]|}\, 
				\Delta \downarrow \Delta' $}
			\RightLabel{$ \scriptsize \textsc{i-if}$}
			\UnaryInfC{$\mbox{\verb|inv[if[$ g $,$ z $,$ s $]]|}\, 
				\Delta \downarrow \Delta'$}
			\DisplayProof			
			\qquad
			\AxiomC{$\mbox{\verb|it[inv[$ f $]]|}\,
				\Delta \downarrow 	\Delta'$}
			\RightLabel{$ \scriptsize \textsc{i-it}$}
			\UnaryInfC{$\mbox{\verb|inv[it[$ f $]]|}\,
				\Delta \downarrow 	\Delta'$}
			\DisplayProof			
			\\[0.5cm]
			\AxiomC{$ v < 0 $}
			\AxiomC{$f\Delta_f \downarrow \Delta'_f $}
			\AxiomC{$\texttt{it}[f](\Delta'_f \cdot [x : v+1]) 
				\downarrow 
				(\Delta''_f \cdot [x : v+1]) $}
			\RightLabel{$ \scriptsize \textsc{i-its}$}
			\TrinaryInfC{$\texttt{it}[f](\Delta_f \cdot [x : v])
				\downarrow (\Delta''_f \cdot [x : v])$}
			\\
			\AxiomC{$f\Delta \downarrow \Delta'$}
			\RightLabel{$ \scriptsize \textsc{i-inv}$}
			\UnaryInfC{$ \mbox{\verb|inv[inv[$ f $]]|}\Delta \downarrow \Delta' 
				$}
			\DisplayProof			
			\qquad
			\AxiomC{$\mbox{\verb|inv[$ \Gamma(f) $]|}\Delta 
				\downarrow \Delta' $}
			\RightLabel{$ \scriptsize \textsc{i-fcall}$}
			\UnaryInfC{$\mbox{\verb|inv[$ f $]|}\Delta 
				\downarrow \Delta' $}
			\DisplayProof			
			\\[0.25cm]
		\end{tabular}
	}
	\caption{The single-relation big-step operational semantics of 
		\textsf{Yarel} that defines the behaviour of \verb|inv|.}
	\label{figure:Single-relation big-step operational semantics of Yarel: 
		second part}
\end{figure}

Figure~\ref{figure:Single-relation big-step operational semantics of Yarel: 
second part} introduces the operational semantics of \verb|inv|. The whole set of rules internalizes the existence of the inverse of any given function  we define in \textsf{Yarel}.

As an example, let us look at how \verb|inv| works, by applying \verb|sub| to $ [x:2, y:1] $, the goal being calculating  $ 2 - 1 $. 
The derivation is:
\begin{equation}
\label{equation:inv[sub] SOS derivation}
\hspace{-2.5cm}
 \scalebox{.7}{
  \begin{minipage}{\linewidth}
  	\begin{prooftree}
        \AxiomC{$  $}
  		\RightLabel{$ \scriptsize \textsc{dec}$}
  		\UnaryInfC{$\mbox{\verb|dec|}[x:2]\downarrow [x:1]\ $}
        \RightLabel{$ \scriptsize \textsc{inv}$}
        \UnaryInfC{$\mbox{\verb|inv[inc]|}[x:2]\downarrow [x:1]\ $}

        \AxiomC{$  $}
        \RightLabel{$ \scriptsize \textsc{dec}$}
        \UnaryInfC{$\mbox{\verb|dec|}[y:1]\downarrow [y:0]\ $}

  		\RightLabel{$ \scriptsize \textsc{par}$}
        \BinaryInfC{$\mbox{\verb+(inv[inc]|dec)+}[x:2,y:1] \downarrow [x:1, y:0] $}
  		
  		\AxiomC{$ $}
  		\RightLabel{$ \scriptsize \textsc{itz}$}  		
  		\UnaryInfC{$\mbox{\verb|it[inv[inc]]|}
              [x:1, y:0] \downarrow [x:1, y:0] $}
  		
  		\RightLabel{$ \scriptsize \textsc{seq}$}
  		\BinaryInfC{$\mbox{\verb+(inv[inc]|dec);it[inv[inc]]+}
  			[x:2, y:1] 
  			\downarrow [x:1, y:0]$}
  		
  		\RightLabel{$ \scriptsize \textsc{itg}$}
        \UnaryInfC{$\mbox{\verb|it[inv[inc]]|}[x:2, y:1] 
	    \downarrow [x:1, y:1]$}

  		\RightLabel{$ \scriptsize \textsc{i-it}$}
        \UnaryInfC{$\mbox{\verb|inv[it[inc]]|}[x:2, y:1] 
	        \downarrow [x:1, y:1]$}

  		\RightLabel{$ \scriptsize \textsc{i-fcall}$}
        \UnaryInfC{$\mbox{\verb|inv[sub]|}[x:2, y:1] 
        	\downarrow [x:1, y:1]$}
  	\end{prooftree}
  \end{minipage}
 }
\end{equation}
\noindent
The occurrence of $ \textsc{i-fcall} $ in~\eqref{equation:inv[sub] SOS derivation} is an instance of the namesake rule in Figure~\ref{figure:Single-relation big-step operational semantics of Yarel: second part}. Like for $ \textsc{fcall} $, it relies on the assumption that a 
\emph{look-up table} $ \Gamma $ exists able to associate names of functions to
the corresponding body, in accordance with definitions \verb|def| and 
declarations \verb|dcl| already met in the module. So, it replaces \verb|sub| with its definition \verb|it[inc]|.

The occurrence of $ \textsc{i-it} $ in~\eqref{equation:inv[sub] SOS derivation} 
is an instance of the namesake rule in Figure~\ref{figure:Single-relation big-step operational semantics of Yarel: second part}. It says that \emph{the 
inverse of an iteration of $ f $ is the iteration of the inverse of $ f $}, so we can resume to the operational rules in Figure~\ref{figure:Single-relation big-step operational semantics of Yarel: first part} and apply $ \textsc{itg} $ where \verb|inv| in \verb|inv[inc]| plays no role.
On the other branch of the derivation, \textsc{i-inc} is a base case in the definition of the behavior of \verb|inv|. Other base cases, which let \verb|inv| disappear from the conclusion of a rule to its assumptions are the rules \textsc{i-id}, \textsc{i-neg}, \textsc{i-dec}, \textsc{i-}$\chi$, \textsc{i-seq} and \textsc{i-inv}. In all the remaining rules, we can say that the inverse of a composite function is that function applied to the inverses of its components.

